Power of Bonus in Pricing for Crowdsourcing

We consider a simple form of pricing for a crowdsourcing system, where pricing policy is published a priori, and workers then decide their task acceptance. Such a pricing form is widely adopted in practice for its simplicity, e.g., Amazon Mechanical Turk, although additional sophistication to pricing rule can enhance budget efficiency. With the goal of designing efficient and simple pricing rules, we study the impact of the following two design features in pricing policies: (i) personalization tailoring policy worker-by-worker and (ii) bonus payment to qualified task completion. In the Bayesian setting, where the only prior distribution of workers' profiles is available, we first study the Price of Agnosticism (PoA) that quantifies the utility gap between personalized and common pricing policies. We show that PoA is bounded within a constant factor under some mild conditions, and the impact of bonus is essential in common pricing. These analytic results imply that complex personalized pricing can be replaced by simple common pricing once it is equipped with a proper bonus payment. To provide insights on efficient common pricing, we then study the efficient mechanisms of bonus payment for several profile distribution regimes which may exist in practice. We provide primitive experiments on Amazon Mechanical Turk, which support our analytical findings.

==> analysis.tex <==
% !TEX root =  main.tex

\section{Proofs}
\label{sec:proof}

% We present the complete proofs of all theorems in the previous section.

\subsection{Proof of Theorems}
\paragraph{Proof of Theorem~\ref{thm:hardness}}
To prove, we consider deterministic worker profiles, i.e., $\prob{({s}_i,{c}_i) = (\bar{s}_i,\bar{c}_i)~\forall i \in \set{N}}~=~1$ for some $[(\bar{s}_i, \bar{c}_i)]$. Since it is a special case of our problem, it is sufficient to show that {\perpriceprob} is NP-hard even on this simple setup.
Consider 
the following generalized 0-1 knapsack problem ({GKP}): for $\vec{s}, \vec{c} \in \mathbb{R}^n$,
% \vspace{-0.2cm}
% \separator
% \vspace{-0.2cm}
\begin{subequations} \label{eq:GKP}
\begin{align}
\text{\hspace{-1cm}\bf GKP:} \quad 
\underset{\vec{x}\in \{0,1\}^n}{\textnormal{maximize}}  & \quad
u(\vec{{s}} \circ \vec{x} ) \nonumber  \\
  \textnormal{subject to} & \quad
  \sum_{i=1}^{n}{c}_ix_i\leq B \;. \label{eq:GKP-condi}
\end{align}
\end{subequations}
% \separator
It is well-known that {GKP} with a additive $u(\cdot)$ is NP-hard \cite{Knapsack:Dantzig}.
We now show that (i) if $[p_i^\star]$ is a solution of {\perpriceprob} in (4), then a solution of GKP in \eqref{eq:GKP} is given as 
$[(\phi_i(p^\star_i)\})]$ in (1), and (ii) if $[(x_i^\star)]$ is a solution of GKP, then a solution of {\perpriceprob} is given as $p_i = c_i \cdot x_i.$ We prove (i) and (ii) by contradiction. 

\noindent{\em (i).} Let $\vec{x}^\star = \{\phi_i(p_i^\star)\}_{i \in \set{N}}$,
where $p^\star = \{p_i^\star\}_{i \in \set{N}}$ is the solution of {\perpriceprob}, i.e., utility of $p^\star$ is $u(\vec{s} \circ \vec{x}^\star)$.
Then it is straightforward to check that $\vec{x}^\star$ satisfies the constraint in \eqref{eq:GKP-condi}.
Suppose $\vec{x}^\star$ is not a solution of GKP
so that there exists a solution $\vec{x}'$ such that $u(\vec{s} \circ \vec{x}') > u(\vec{s} \circ \vec{x}^\star)$.
We now construct a {\perprice} $\pi' = \{c_i x'_i\}_{i \in \set{N}}$ from $\vec{x}'$.
 Since $\vec{x}'$ is a solution of GKP, pricing $\pi'$ satisfies the constraints in (2).
 The construction of ${\pi}'$ contradicts the optimality of $\pi^\star,$
 since the utility of $\pi'$ is strictly larger than that of $\pi^\star$.

\noindent{\em (ii).} Let $[(x_i^{\star})]$ be an optimal solution of GKP. Let $[p_i]$ be a solution of {\perpriceprob} such that $u(\vec{s} \circ [p_i]) > u(\vec{x} \circ \vec{x}^\star)$. We now construct an allocation vector $x' = [(\mathbbm{1}[p_i(s_i) \geq c_i])]$ from personalized pricing $[p_i]$. Since $[p_i]$ is budget-feasible, it is straightforward that $x'$ is a feasible solution of GKP, which again contradicts the optimality of $[(x^\star)]$, and it completes the proof. \ep

\paragraph{Proof of Theorem~\ref{thm:ex_post}} 
We first lay out the foundations in defining the ex-ante budget constraint as follows:
For $B \ge 0$ and 
$\pi \in \set{F}(B):= \{\pi : 
\sum_{i\in \set{N}} \expect{(p_i(s_i)
\mathbbm{1}[p_i(s_i) > c_i ]} \leq B
\}$,
let $\set{Q}(p, B)$ be the distribution of 
random vector $\vec{y} \in \{0,1\}^{\set{N}}$ 
consisting of $y_i = \max \big\{ \mathbbm{1}[p_i(s_i) > c_i ],
\mathbbm{1}[p_i(s_i) = c_i] b_i \big\}.$
% \begin{multline}
% \label{eq:ex_ante_allocation}
% y_i = \max \Big\{ \mathbbm{1}[p_i+q_i(s_i) > c_i ], \cr 
% \mathbbm{1}[p_i+q_i(s_i) = c_i] b_i \Big\},
% \end{multline}
Here, $b_i$ is an independent Bernoulli random variable with parameter $\rho (\pi, B)$, where 
\begin{align*} 
\rho(\pi,B) := \min\left\{1, 
\frac{B-\sum_{i \in {\mathcal N}} \mathbb{E} [(p_i(s_i)) \mathbbm{1}[p_i(s_i) > c_i]]}{\sum_{i \in {\mathcal N}} \mathbb{E}[(p_i(s_i)) \mathbbm{1}[p_i(s_i) = c_i]]}
\right\}  \;.
\end{align*}
Note that $\rho(p,B)\geq 0$ directly comes from the definition of $\pi$.
% Note that $\rho (\pi, B) \ge 0$
% for $\pi \in {\mathcal F}(B)
% := \{\pi : 
% \sum_{i\in {\mathcal N}} \mathbb{E}[(p_i+q_i(s_i))
% \mathbbm{1}[p_i+q_i(s_i) > c_i ]] \leq B
% \}

% \begin{align} \label{eq:ex_ante_parameter}
% \rho(\pi,B) \defeq \frac{B-\sum_{i \in \set{N}} \expect{(p_i+q_i(s_i)) \mathbbm{1}[p_i+q_i(s_i) > c_i]}}{\sum_{i \in \set{N}} \expect{(p_i+q_i(s_i)) \mathbbm{1}[p_i+q_i(s_i) = c_i]}}.
% \end{align}
Thanks to the generation of $\vec{y} \sim \set{Q}(\pi,B)$
and condition on $\pi \in \set{F}(B)$,
the task allocation according to $\vec{y}$ 
verifies budget constraint in expectation sense:
\begin{align*} \textstyle
      \EXP_{\vec{y} \sim \set{Q}(p,B)} \big[
      \sum_{i \in \set{N}}
      (p_i(s_i)) y_i \big] \le B ,
\end{align*}
which is also known as 
{\em ex-ante} budget constraint.
We then formulate an ex-ante version of {\OPP}$(B)$ in \eqref{eq:opt_goal} as follows:
\begin{align}
\text{\hspace{-0.2cm} {\bf OPP-E}$(B)$:} \quad
\underset{p \in \set{F}(B)}{\textnormal{maximize}}  & \quad
V(B; p) \label{eq:ex_ante_object} 
\end{align}
where $V(B; p) := \EXP_{\vec{y} \sim \set{Q}(p, B)} [ U(\vec{s} \circ \vec{y} )]$. 

We consider a common pricing that has {\bf \em linear bonus with zero base payment,} which we call {\bf LBZB} pricing and  denote by
$\linear(\alpha)$ with the slope $\alpha \ge 0$, i.e., $p_c(\alpha) := \alpha s$. 
Next we define a constant $\alpha_B$ as the following:
\begin{align*}
&\alpha_{B} \defeq \inf \left\{ \alpha \ge 0 : 
\sum_{i \in \set{N}}\EXP 
\big[ c_i z_i (\alpha, \rho)  \big]  \geq B,
~\exists \rho \in [0,1]\right\},
\end{align*}
for a random variable $z_i$ defined as
$z_i(\alpha, \rho) \defeq \mathbbm{1}[\alpha u_0(s_i) > c_i]
+\rho \mathbbm{1}[\alpha u_0(s_i) = c_i].$
Now we prove that $p_c(\alpha_B)$ achieves the approximation ratio stated in the theorem.


\smallskip
We present two key lemmas whose proofs are in Section~\ref{sec:lemma}. \begin{lemma}[Ex-ante PoA]\label{lem:apx_ante} 
Given a budget $B$, the LBZB pricing {\linpol}$(\alpha_B)$ is $(1,\mu_B)$-approximate of $\text{OPP-E}(B)$, where $\mu_B$ is defined as follows:
\begin{align*}
& \mu_B \defeq  \frac{\sum_{i \in \set{N}}\EXP \big[  \alpha_B s_i z_i(\alpha_B, \lambda_B)
\big] }
{\sum_{i \in \set{N}}\EXP  [ c_i z_i(\alpha_B, \lambda_B)]},  \quad \text{where}\\
&\lambda_B \defeq \inf \left\{ \lambda\in [0,1] : 
\sum_{i \in \set{N}}\EXP 
\big[ c_i z_i (\alpha_B, \lambda)  \big]  \geq B \right\}.
\end{align*}
\end{lemma}  
\begin{lemma}[Connection to ex-post]\label{lem:post_to_ante}
For sufficiently large $n$, 
if $B =\Omega(n)$,
 for a separable $u(\cdot)$ and the LBZB pricing $\linear(\alpha_B),$ we have 
%the following under any worker arrival order: 
\begin{align*}
U\!\Big(\mu_{B} B; \linear(\alpha_{B}) \Big) 
\ge \Big(1-O\left(e^{-n^{1/6}}\right)\Big) V\!\Big(\mu_B B ; \linear(\alpha_B) \Big) .
\end{align*}
\end{lemma}

Lemma~\ref{lem:apx_ante} provides an approximation ratio of $\linear(\alpha_B)$ to OPP-E$(B)$.
We then use Lemma~\ref{lem:post_to_ante} to translate 
the ex-ante approximation into the ex-post one, where for sufficiently large $n$ and $B$, we have
\begin{align*}
U\!\Big(\mu_{B} B; \linear(\alpha_{B}) \Big) 
&\ge \Big(1-O(e^{-n^{1/6}})\Big) V\!\Big(\mu_B B ; \linear(\alpha_B) \Big) \\
&\ge \Big(1-O(e^{-n^{1/6}})\Big) V^\star(B),
\end{align*}
where we use Lemmas~\ref{lem:apx_ante}~and~\ref{lem:post_to_ante} for the first and last inequalities, respectively. This concludes the proof since $\pi^\star_p(B) \in \set{F}(B)$, i.e., $V^\star(B) \ge U\big(B;\pi^\star_p(B)\big)$. One can easily check that $\mu_B = O(1)$ by the correlation assumption.

\paragraph{Observation on LBZB}
We provide a couple of interpretations of LBZB introduced in the proof of Theorem~\ref{thm:ex_post}. 
We note that the linear bonus in the LBZB pricing $\linear(\alpha)$ recruits only {\em efficient} workers whose utility-to-cost ratio $s_i/c_i$ is at least $1/\alpha$, i.e., $x_i = 1$  only if $s_i / c_i \ge {1}/{\alpha}$.
A good personalized pricing may also target such efficient workers in priority, while user-agnosticity of the common pricing pays more often than the personalized one. Hence, the simple common pricing $\linear(\alpha)$ with a good choice of $\alpha = \alpha_B$ and more budget $(O(1) \times B)$ achieves at least $1 - o(1)$ of the optimal utility of {\perpriceprob}$(B)$. 

For the employed LBZB common pricing to be practical, it is required that $\alpha_B$ allows easy computation, which turns to be polynomial-time computable with respect $n.$ To do so, 
given all the distributions of worker profiles, 
it is enough to find $\alpha$ such that $\sum_{i \in \set{N}}\EXP \big[c_i \mathbbm{1}[\alpha s_i \geq c_i] \big] \geq B$ and $\sum_{i \in \set{N}}\EXP \big[c_i \mathbbm{1}[\alpha s_i > c_i] \big] \leq B$, where of each term in the summations can be computed in $O(1)$ time. Since the available interval of $\alpha$ is bounded, using some root finding algorithms, we can find such $\alpha$ approximately in at most $c \cdot O(1) \cdot 2n$ time for some constant $c$.






%\vspace{-0.3cm}



\paragraph{Proof of Theorem~\ref{thm:pad_bonus}}
For a given budget $B$, we denote $u^\star(B)$ and $u_0^\star(B)$ to be the utilities of an optimal pricing by solving $\text{OPP}(B)$, and an optimal common pricing without bonus, respectively.
Since $u_0$ is not a zero function, we can find $s_0$ such that $u_0(s_0)>0$.
Given a budget $B$, we also can find $c_0$ such that $c_0n > B$.
Now, for $\varepsilon = \frac{B}{n^2c} < 1$, consider the following profiles of $n$ workers:
\begin{subnumcases}{\label{eq:eg-profile}(s_i, c_i) =}
   (s_0, c_0) & if $0 < i \leq \varepsilon n$  \nonumber\\
 (0, c_0)  &  if $\varepsilon n < i \leq n$.  \nonumber
\end{subnumcases}
For simplicity, we assume that $\varepsilon n$ is an integer without loss of generality.
Then, it is straightforward to check that $u^\star(B) = \varepsilon n u_0(s)$.
Now we compute the optimal utility for pricing without personalization nor bonus under the worst-case worker arrival model. Consider a scenario where all the spammers arrive ahead of the hammers. We assume that the budget is augmented by a factor $\delta = o(n)$. Then, the total payment to spammers is computed as the following:
\begin{align*}
(1-\varepsilon)cn = nc-B/n \geq \delta B,
\end{align*}
where the inequality comes from that $\delta = o(n)$. Hence, the optimal common pricing without bonus failed to recruit any hammers, and it concludes the proof.


\subsection{Proof of Lemmas}
\label{sec:lemma}

\paragraph{Proof of Lemma~\ref{lem:apx_ante}}
We prove that $V(\mu_B B ; \linear(\alpha_B))$ exactly achieves the optimum of ex-ante mechanism given budget $B$, i.e., $V(\mu_B B ; \linear(\alpha_B)) \geq V^\star(B)$.
First, since $u_0(s_i)/c_i$ is also a positive random variable, 
it is straightforward to have that the right-continuity of CDF of $u_0(s_i)/c_i$ implies that $\expect{c_i z_i(\alpha_B, \rho_B)} = B$.
We now consider the following relaxed version of the ex-ante mechanism.
\begin{align*}
\text{\hspace{-0.2cm} {\bf Oracle}$(B)$:} \quad
\underset{\vec{x}= [(x_i(s_i,c_i))]\in [0,1]^n}{\textnormal{maximize}}  & \quad
\sum_{i \in \set{N}}\EXP \left[ u(s \circ x)) \right]  \\
\quad \text{\hspace{-0.2cm} s.t.}\quad & \quad
\sum_{i \in \set{N}} \EXP \left[ c_ix_i \right] \leq B.
\end{align*}
Note that $\vec{x}$ is not necessarily sampled from $\set{Q}(\vec{\pi},B)$, so that the domain of $\vec{x}$ is also extended to any real number in $[0,1]^n$. It is trivial that the optimum of \textbf{Oracle}($B$) is dominant to that of ex-ante mechanism given budget $B$.
We show that the allocation vector obtained by common pricing $\linear(\alpha_B)$ under ex-ante mechanism becomes optimal for \textbf{Oracle}($B$).
We first introduce two lemmas that are useful in the proof whose proofs are presented in the end of this section.

\begin{lemma}\label{lem:1}
Let $\vec{z}^\star$ be any optimal allocation vector for \textbf{Oracle}($B$). The following holds for any random incidence of random vector $(\vec{s}, \vec{c})$.
\begin{compactenum}[(i)]
\item If $\alpha_B u_0(s_i) < c_i$, then $z_i^\star(s_i,c_i) = 0 $ a.e. for any $i \in \set{N}$.
\item If $\alpha_B u_0(s_i) > c_i$, then $z_i^\star(s_i,c_i) = 1 $ a.e. for any $i \in \set{N}$.
\end{compactenum}
\end{lemma}

% \begin{lemma}\label{lem:2}
% Let $\vec{z}^\star$ be any optimal allocation vector for \textbf{Oracle}($B$). If $\alpha_B u_0(s_i) > c_i$, then $z_i^\star(s_i,c_i) = 1 $ a.e. for any $i \in \set{N}$.
% \end{lemma}
\begin{lemma}\label{lem:3}
For $i \in \set{N},$ let $\set{H}_i = \left\{(s_i,c_i) | \alpha_B s_i = c_i \right\}$. Let $\vec{x}$ and $\vec{x}'$ be the two allocation vectors which satisfies 
$\sum_{i \in \set{N}} \EXP_{(s_i,c_i) \in \set{H}_i} [c_ix_i] = \sum_{i \in \set{N}} \EXP_{(s_i,c_i) \in \set{H}_i} [c_ix_i']. $ 
Then, the achieved utilities by $\vec{x}$ and $\vec{x}'$ are equal, i.e., 
$$
\sum_{i \in \set{N}} \EXP_{(s_i,c_i) \in \set{H}_i} [u_0(s_i)x_i] = \sum_{i \in \set{N}} \EXP_{(s_i,c_i) \in \set{H}_i} [u_0(s_i)x_i']. 
$$
\end{lemma}
Let $\vec{\chi}$ be the allocation vector induced by $\linear(\alpha_B)$ under the augmented budget $\mu_B B$.
By Lemma~\ref{lem:1}, it is straightforward to check that optimal allocation vector $\vec{z}^\star$ must recruit worker $i$ if $\alpha_B s_i > c_i$, and must reject her if $\alpha_B s_i < c_i$.
We first consider the scenario where only allocating the budget to workers with $\alpha_B s_i > c_i$ fully exhaust the budget $B$.
In this case, $\sum_{i \in \set{N}} \expect{c_iz_i^{\star} \mathbbm{1}[\alpha_B u_0(s_i) > c_i]}= B$, and it implies that $\vec{\chi}$ is exactly the same as $\vec{z}$ by the definition of $\alpha_B$.
Moreover, the expected payment to workers in $\linear(\alpha_B)$ can be computed as:
\begin{equation*}
\sum_{i \in \set{N}} \EXP [\alpha_B u_0(s_i)z_i(\alpha_B, \lambda_B)]
= \sum_{i \in \set{N}} \bexpect{\alpha_B u_0(s_i) \mathbbm{1}[\alpha_B u_0(s_i) > c_i]} = \mu_B B,
\end{equation*}
which guarantees that $\linear(\alpha_B)$ is $\mu_B B$-budget feasible, and concludes the proof.
We now suppose that the budget is not exhausted, hence optimal allocation vector must recruit some workers with $\alpha_B u_0(s_i) = c_i$ (workers at boundary),
i.e.,  $\sum_{i \in \set{N}} \EXP [c_iz_i^{\star} \mathbbm{1}[\alpha_B u_0(s_i) > c_i]] < B$.
By the definition of $\alpha_B$ and $\lambda_B$, the following holds:
\begin{align*}
\sum_{i \in \set{N}} \EXP [c_i \chi_i\mathbbm{1}[\alpha_B u_0 = c_i]] &= \sum_{i \in \set{N}} \EXP[c_i \mathbbm{1}[\alpha_B u_0 = c_i]]\cdot \rho(\linear(\alpha_B), \mu_B B)\\
&=\sum_{i \in \set{N}} \EXP[c_i \mathbbm{1}[\alpha_B u_0 = c_i]] \cdot
 \frac{\mu_B B -\sum_{i \in \set{N}} \EXP [\alpha_B u_0(s_i) \mathbbm{1}[\alpha_B u_0(s_i) > c_i]]}
{ \sum_{i \in \set{N}} \EXP[\alpha_B u_0(s_i) \mathbbm{1}[\alpha_B u_0 = c_i]]}\\
&= B- \sum_{i \in \set{N}} \EXP [\alpha_B u_0(s_i) \mathbbm{1}[\alpha_B u_0(s_i) > c_i]].
\end{align*}
Moreover, it is straightforward to see that any optimal allocation vector $z^\star$ must exhaust the budget in workers with $\alpha_B s_i = c_i$, i.e., 
\begin{equation*}
\sum_{i \in\set{N}}\EXP [ c_i z_i^\star \mathbbm{1}[\alpha_B u_0(s_i) = c_i]] 
= B - \sum_{i \in\set{N}}\EXP [ c_i z_i^\star \mathbbm{1}[\alpha_B u_0(s_i) > c_i]].
\end{equation*}
Hence by Lemma~\ref{lem:3}, we have:
\begin{eqnarray}
\sum_{i \in \set{N}} \EXP_{(s_i,c_i) \in H_i} [u_0(s_i)\chi_i] = \sum_{i \in \set{N}} \EXP_{(s_i,c_i) \in H_i} [u_0(s_i)z_i^\star], \label{thm:1}
\end{eqnarray}
which implies that the expected utility gain from workers at boundaries, i.e. workers satisfying $\alpha_B u_0(s_i) = c_i$, is exactly the same between two allocation vectors $\vec{z}^\star$ and $\vec{\chi}$. We can also show that $\linear(\alpha_B)$ is $\mu_B B$-budget feasible in this scenario.
Finally, combining Lemma~\ref{lem:1} and \eqref{thm:1}, 
we complete the proof of Lemma~\ref{lem:apx_ante}. \ep



\paragraph{Proof of Lemma~\ref{lem:post_to_ante}}
We first borrow the following two theorems provided by \cite{proof:Vondrak11} and \cite{Posted:Balkanski16}.
\begin{theorem}[\cite{proof:Vondrak11}]
\label{thm:vondrak10}
Given $\epsilon \in (0,\frac{1}{2})$, $k > 2/\epsilon$, and pricing $\pi$ under budget $B$, we denote a payment of worker $i$ as a random variable $p_i \in [0,\frac{B}{k}]$ (k-large market) where $p_i$'s are mutually independent.
If $p_i$ satisfies $\sum_i \expect{p_i} \leq (1-\epsilon)B$ (scaled ex-ante budget feasible), 
then the probability that the sum of costs of selected agents does not exceed the budget less the cost
of any agent, i.e. $\prob{\sum_{i \in \set{N}}p_i \leq (1-1/k)B}$, is at least $1-e^{-\epsilon^2(1-\epsilon)k/12}$.
\end{theorem}
\begin{theorem}[\cite{Posted:Balkanski16}] \label{thm:balkanski}
 Given the same condition in $k,\varepsilon$, for given worker arrival order $\sigma$ and pricing policy $\pi$ with scaled ex-ante budget constraint, i.e. $\sum_{i \in \set{N}} \expect{p_i+q_i(s_i)} \leq (1-\varepsilon)B$, and k-large market condition, i.e. $p_i+q_i(s_i) \leq B/k$, then the probability that a worker is offered her price is at least, $\prob{\sum_{i \in \set{N}} p_i+q_i(s_i) \leq (1-1/k)B}$.
\end{theorem}
% \note{is this really needed?}
% Firstly, if $\sum_{i \in \set{N}} c_{\max} \leq \mu_B B$, then the result trivially holds. Hence, we suppose that $\sum_{i \in \set{N}} c_{\max} > \mu_B B$ in the remainder of this proof.
% We will use Theorem~\ref{thm:vondrak10} for which we now verify the condition of $k$-large market, and scaled ex-ante budget feasibility with $\mu_B B',$ where $B' = \frac{\mu_B B}{1-\varepsilon}$. 
% The total expected payment to workers in $\linear(\alpha_B)$ is computed as:
% \begin{multline*}
% \sum_{i \in \set{N}}  \Bigg( \bexpect{\alpha_B u_0(s_i) \mathbbm{1}[\alpha_B u_0(s_i) > c_i]} 
% \cr +\rho(\pi, B)\bexpect{\alpha_B u_0(s_i) \mathbbm{1}[\alpha_B u_0(s_i) = c_i]} \Bigg) \leq \mu_B B,
% \end{multline*}
% where in terms of $B'$, $\linear(\alpha_B)$ satisfies the scaled ex-ante budget feasibility.
% Suppose $\alpha_Bu_0(s_{\min}) > c_{\min}$.
% Then the total expected payment to workers in $\linear(\alpha_B)$ is given by: 
% \begin{align*}
% \mu_B B &\geq \sum_{i \in \set{N}} \bexpect{\alpha_Bu_0(s_i) \mathbbm{1}[\alpha_Bu_0(s_i) > c_i]}\cr
% &= \sum_{i \in \set{N}} \expect{\alpha_Bu_0(s_{\min})}  \geq n\cdot c_{\max},
% \end{align*}
% which is a contradiction and we conclude that $\alpha_Bu_0(s_{\min}) \leq c_{\max}$. 
% By the assumption in $s_{\max}$, the expected payment to any worker $i$ satisfies the following inequality:
% \begin{eqnarray}
% \alpha_B u_0(s_{\max}) \leq \frac{\mu_B B}{n^{5/6}} \leq \frac{\mu_B B'}{n^{5/6}}
% \end{eqnarray}
Putting $k=n^{1/2}$ and $\varepsilon = n^{-1/6}$, it is straightforward to check that it satisfies k-large market condition and scaled ex-ante budget constraint by assumption.
Hence by Theorem~\ref{thm:vondrak10}, ex-post mechanism with pricing $\linear(\alpha_B)$ satisfies the following:
\begin{equation*}
\bprob{\sum_{i \in \set{N}} \alpha_Bu_0(s_i) \leq (1-n^{-5/6}) B'}  \geq 1-e^{(n^{-1/6}-n^{1/6})/12} = 1-O(e^{-n^{1/6}}).
\end{equation*}
Finally, we get the following expected ex-post utility of pricing $\linear(\alpha_B)$, which completes the proof.

\begin{align*}
U(\mu_B B;\linear(\alpha_B))&=\EXP_{\vec{x}\sim\set{P}(B,\linear(\alpha_B))}[u(\vec{s} \circ \vec{x} )]
= \sum_{i \in \set{N}}\expect{u_0(s_i) \cdot x_i } \cr
&\geq \sum_{i \in \set{N}}\bexpect{u_0(s_i) \cdot \mathbbm{1}[\alpha_B u_0(s_i) \geq c_i] }\bprob{\sum_{i \in \set{N}} \alpha_Bu_0(s_i) \leq (1-n^{-5/6}) B'} \\
&\geq \sum_{i \in \set{N}}\bexpect{u_0(s_i) \cdot \mathbbm{1}[\alpha_B u_0(s_i) \geq c_i] } \lf(1-O(e^{-n^{1/6}}) \ri)\\ 
&\geq \big(1-O(e^{-n^{1/6}}) \big)V(\mu_B B; \linear(\alpha_B)).
\end{align*} \ep

% \paragraph{Proof of Lemma~\ref{lem:1} and ~\ref{lem:3}}
% To prove Lemma~\ref{lem:1}, we first claim that if the statement (i) is false, then (ii) is also false, and vice versa. In next, we assume that there exists two random incidences which contradicts (i) and (ii), respectively, then construct new allocation vector by changing its behavior on that two random incidences whereas keeping being consistent as $\vec{z}^\star$ otherwise. Then we prove that such allocation vector is feasible in {\bf Oracle}($B$) and its utility dominate that of $\vec{z}^\star$, which is a contradiction to the assumption that $\vec{z}^\star$ is the optimal solution.
% We provide the detailed proof of both lemmas in our technical report~\cite{techreport} due to the space limit.

\paragraph{Proof of Lemma~\ref{lem:1}}
The underlying intuition is that greedy algorithm outputs the exact optimum of the {\em fractional} knapsack problem.
We use proof by contradiction. 
Let the sample space of the random vector $(s_i, c_i)$ be $O_i$. 
We define the following two sets.
\begin{eqnarray*}
\set{E}_i := \{ (\vec{s}, \vec{c}) \; | \; \alpha_B u_0(s_i) < c_i, z_i^\star(\vec{s}, \vec{c}) > 0 \}\\
\set{F}_i := \{ (\vec{s}, \vec{c}) \; | \; \alpha_B u_0(s_i) \geq c_i, z_i^\star(\vec{s}, \vec{c}) < 1 \}\\
\set{G}_i := \{ (\vec{s}, \vec{c}) \; | \; \alpha_B u_0(s_i) \geq c_i, z_i^\star(\vec{s}, \vec{c}) = 1 \}.
\end{eqnarray*}
Note that given any optimal allocation vector $z^\star(\vec{s}, \vec{c})$, $E_i$ denotes the set of all incidences of random vector $(\vec{s}, \vec{c})$ that satisfies $\alpha_B u_0(s_i) < c_i$ and $z^\star_i(\vec{s}, \vec{c}) > 0$.
Firstly, we claim that if there exists $i \in \set{N}$ such that $\bprob{\set{E}_i} > 0,$ then 
there exist $j \in \set{N}$ such that $\bprob{\set{F}_j} > 0$.
Suppose not, i.e. $\bprob{\set{E}_i} > 0$ for $i \in \set{N}$, and $\bprob{\set{F}_j} = 0$ for any $j \in \set{N}$.
By assumption, we get $\bprob{\set{G}_j} = \bprob{\mathbbm{1} [\alpha_B u_0(s_i) \geq c_i]}$.
Since $\set{E}_i$, $\set{F}_i$, and $\set{G}_i$ are mutually exclusive, the expected payment to workers in $\vec{z}^\star$ satisfies the following inequalities:
\begin{align}
B&\geq \sum_{i \in \set{N}} \EXP_{(s_i,c_i) \in \set{E}_i} [c_i z_i^\star] + \EXP_{(s_i,c_i) \in \set{F}_i} [c_i z_i^\star] + \EXP_{(s_i,c_i) \in \set{G}_i} [c_i z_i^\star] \\
&\geq \sum_{i \in \set{N}} \EXP_{(s_i,c_i) \in \set{E}_i} [c_i z_i^\star]  + \EXP_{(s_i,c_i) \in \set{G}_i} [c_i z_i^\star] \\
&\geq \sum_{i \in \set{N}}\EXP_{(s_i,c_i) \in \set{E}_i} [c_i z_i^\star]  + \EXP [c_i \mathbbm{1}[\alpha_B s_i \geq c_i]]  \\
&\geq B + \sum_{i \in \set{N}}\EXP_{(s_i,c_i) \in \set{E}_i} [c_i z_i^\star] > B,
\end{align}
which is a contradiction.
Hence we conclude that if there exists $i \in \set{N}$ with $\bprob{\set{E}_i} > 0,$ then there exists $j \in \set{N}$ with $\bprob{\set{F}_j} > 0$.
By our claim, we can choose two random incidences $(\bar{s_i}, \bar{c_i}) \in \set{E}_i$ and $(\tilde{s_j},\tilde{c_j}) \in \set{F}_j$, which are $i$-th and $j$-th element in incidences of random vector $(\bar{\vec{s}}, \bar{\vec{c}})$ and $(\tilde{\vec{s}}, \tilde{\vec{c}})$, respectively.
Now we construct an allocation vector $\vec{y} \in [0,1]^n$, which is equal to $\vec{z}^\star$ except the two sample points $(\bar{\vec{s}}, \bar{\vec{c}})$ and $(\tilde{\vec{s}}, \tilde{\vec{c}})$ so that $y_j(\tilde{s_j},\tilde{c_j}) = z_j^{\star}(\tilde{s_j}, \tilde{c_j}) + \varepsilon$, and 
$y_i(\bar{s_i}, \bar{c_i}) = z_i^{\star}(\bar{s_i}, \bar{c_i}) - \frac{\tilde{c_j}}{\bar{c_i}}\varepsilon$, where $\varepsilon = \min \left\{ \frac{\bar{c_i}}{\tilde{c_j}}z_i^{\star}(\bar{s_i}, \bar{c_i}) , 1- z_j^{\star}(\tilde{s_j}, \tilde{c_j})  \right\}$.
Then, the difference between the total expected payment to workers in $\vec{y}$ and $\vec{z}^\star$ can be computed as the following:
\begin{align*}
\sum_{i \in \set{N}}\EXP[c_i z_i^\star] - \sum_{i \in \set{N}} \EXP[c_i y_i] &= \left (\tilde{c_j}y_j(\tilde{s_j}, \tilde{c_j}) + \bar{c_i}y_i(\bar{s_i}, \bar{c_i}) \right) -
\left ( (\tilde{c_j}z_j^\star(\tilde{s_j}, \tilde{c_j}) +\bar{c_i}z_i^\star(\bar{s_i}, \bar{c_i}))\right)
\\
&=
\tilde{c_j}(z_j^\star(\tilde{s_j}, \tilde{c_j}) + \varepsilon) + \bar{c_i}(z_i^\star(\bar{s_i}, \bar{c_i})- \frac{\tilde{c_j}}{\bar{c_i}}\varepsilon)-(\tilde{c_j}z_j^\star(\tilde{s_j}, \tilde{c_j}) +\bar{c_i}z_i^\star(\bar{s_i}, \bar{c_i}))
\\
&=
\tilde{c_j}\varepsilon - \bar{c_i}\cdot \frac{\tilde{c_j}}{\bar{c_i}} \varepsilon = 0,
\end{align*}
which implies that $\vec{y}$ is also a feasible point for \textbf{Oracle}($B$). 
Now we compute the difference of expected utility between $\vec{y}$ and $\vec{z}^\star$ as the following:
\begin{align*}
\sum_{i \in \set{N}}\EXP[u_0(s_i)y_i] &- \sum_{i \in \set{N}} \EXP[u_0(s_i) z_i^\star]\\
&=
u_0(\tilde{s_j })(z_j^\star(\tilde{s_j}, \tilde{c_j}) + \varepsilon) + u_0(\bar{s_i })(z_i^\star(\bar{s_i}, \bar{c_i}) -  \frac{\tilde{c_j}\varepsilon}{\bar{c_i}}) - \Big( u_0(\tilde{s_j })z_j^\star(\tilde{s_j}, \tilde{c_j}) +
u_0(\bar{s_i })z_i^\star(\bar{s_i}, \bar{c_i})\Big) \\
&=u_0(\tilde{s_j })\varepsilon -u_0(\bar{s_i })\frac{\tilde{c_j}}{\bar{c_i}}\varepsilon > \frac{\varepsilon}{\alpha_B}(\tilde{c_j} - \bar{c_i}\frac{\bar{c_i}}{\bar{c_i}}) = 0,
\end{align*}
which implies that the expected utility of $\vec{y}$ is strictly larger than $\vec{z}.$ This contradicts the assumption that $\vec{z}$ is optimal solution for \textbf{Oracle}($B$), and it completes the proof of Lemma 4.3. Since the proof for statement (ii) is exactly analogous to that of (i), we omit the detailed proof.\ep

\paragraph{Proof of Lemma~\ref{lem:3}} 
The following inequality directly completes the proof.
% \begin{eqnarray}
% \sum_{i \in \set{N}} \EXP_{(s_i,c_i) \in \set{H}_i} [u_0(s_i)x_i] &=& \sum_{i \in \set{N}} \expect{u_0(s_i)x_i \mathbbm{1}[ \alpha_B u_0(s_i) = c_i]} \\
% &=& \sum_{i \in \set{N}} \bexpect{\frac{c_i}{\alpha_B}x_i \mathbbm{1}[ \alpha_B u_0(s_i) = c_i]} \\
% &=& \sum_{i \in \set{N}} \bexpect{\frac{c_i}{\alpha_B}x_i' \mathbbm{1}[ \alpha_B u_0(s_i) = c_i]}    \label{eq:lem3_3} \\
% &=& \sum_{i \in \set{N}} \EXP_{(s_i,c_i) \in \set{H}_i} [u_0(s_i)x_i'],
% \end{eqnarray}
\begin{align}
\hspace{-0.1cm}\sum_{i \in \set{N}} \EXP_{(s_i,c_i) \in \set{H}_i} [u_0&(s_i)x_i] = \sum_{i \in \set{N}} \expect{u_0(s_i)x_i \mathbbm{1}[ \alpha_B u_0(s_i) = c_i]} 
\label{eq:lem3_1} \\
& =\sum_{i \in \set{N}} \bexpect{\frac{c_i}{\alpha_B}x_i \mathbbm{1}[ \alpha_B u_0(s_i) = c_i]} \label{eq:lem3_2} \\
&= \sum_{i \in \set{N}} \bexpect{\frac{c_i}{\alpha_B}x_i' \mathbbm{1}[ \alpha_B u_0(s_i) = c_i]}    \label{eq:lem3_3} \\
&= \sum_{i \in \set{N}} \EXP_{(s_i,c_i) \in \set{H}_i} [u_0(s_i)x_i'],   
\end{align}
where \eqref{eq:lem3_1} holds from the definition of $\set{H}_i,$ 
and \eqref{eq:lem3_2} and \eqref{eq:lem3_3} holds from our assumption.\ep

\subsection{Proof of Propositions}
\label{sec:propositions}
\paragraph{Proof of Proposition~\ref{prop:1}} 
\paragraph{Proof of Proposition~\ref{prop:2}}
\paragraph{Proof of Proposition~\ref{prop:3}}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> rebuttal.tex <==
%\vspace{-0.23cm}
\section*{Appendix B: Response Report for One-shot revision}
\label{sec:rebuttal}
In what follows, we provide our response to the reviewers' revision requests on paper (\#187) Power of Bonus in Pricing for Crowdsourcing on \textit{2021 Winter Submission deadline}.


First of all, we sincerely thank the reviewers for their valuable and constructive comments, which we believe greatly helped us improve the quality of our
paper. We have revised our manuscript accordingly. 
% In what follows, we provide the summary of our revisions and detailed responses to the reviewers' questions and comments.
We begin with the one-shot revision comments from the TPC chair, most of which cover those of the individual reviewers. Then, for each comment from the individual reviewers, we additionally provide our response or the pointer to our response in the reviewer summary. Throughout this report, for simplicity, we use the following acronym: {\bf RS} (Reviewer Summary from TPC chair) and {\bf REV} (Reviewer).
For each comment, we have indicated the location in the revised manuscript for its corresponding modification.


\subsection*{Review Summary (RS)}
\begin{enumerate}[leftmargin=3.5pt]
\item 

\question{Better integrate this work with prior literature on related pricing approaches in applications such as cloud computing and crowdsourcing.}

\comments{{\bf REV2-(1), REV3-(2)}}

\answer{
As suggested, we have significantly revised Section~\ref{sec:related}  (Related Work).
% completely re-written Paragraph 3,4, and 5 in Section~\ref{sec:related} for more clarity. 
Specifically, in the third paragraph, to reflect {\bf REV3-(2)}, we present the crowdsourcing literature based on principal-agent problem where the workers decide an effort level to exert on the task, and the requester designs a contract to extract costly effort from strategic workers. Compared to those works, we also include some works based on the models that are similar to ours and briefly discuss why these models, where the workers only choose to participate or not, fits to the real-world microtask crowdsourcing platforms.
In the fourth paragraph, we refine the explanation for price discrimination literature.
Finally, in the fifth paragraph, as commented in {\bf REV2-(1)}, we introduce some papers studying on efficient non-discriminatory pricing policy in various real-world applications like ride sharing platform and cloud service platform.
}
   
  {\bf Revision: Page 3, Section~\ref{sec:related}}

\item 
\smallskip
\question{Make it more clear in the theoretic results what forms of pricing are being considered - in particular indicate when a variable such as $p$ represents a policy versus a single price.}

\comments{{\bf REV1-(1), REV1-(3), REV3-(1)}}

\answer{
For the sake of clarity, we have revised the notations and descriptions in our analysis as suggested.
% For Theorem 1 in Section~\ref{sec:poa} and all the propositions in Section~\ref{sec:opt}, we specify the form of pricing policy.
% To briefly summarize the main results, Price-of-Agnosticism analyzes the performance gap between optimal personalized pricing and common pricing, and each propositions in Section~\ref{sec:opt} study the optimal structure of common pricing policy for each profile distribution regime. 
We have also corrected some misleading sentences in abstract and introduction.
}

{\bf Revision: Abstract, Page 2 - Section~\ref{sec:intro}, Page 7 - Section~\ref{sec:poa1}, Page 8,9 - Section~\ref{sec:opt}}

\smallskip
\item 
\question{ Include a more detailed discussion of the limitations/assumption of the crowdsourcing model in the paper. }

\comments{{\bf REV2-(2), REV3-(2), REV3-(3)}}

\answer{
We include more discussions on the limitation and assumption of our model across the paper. To be specific, in Section~\ref{sec:related}, as commented in {\bf REV3-(2)}, 
we provide a justification of assuming that the workers do not strategize their quality after acceptance, but only choose to participate or not with some references.
In Section~\ref{sec:model1}, to address {\bf REV3-(3)}, we discuss how the estimation of ex-post quality can be made in real-world applications, which is apparently inexpensive in most cases. 
% We observe that it can be trivial or not with respect to the requester's task, and one can indirectly estimate the quality even for some non-trivial regimes.
% In paragraph 4, "Worker behavior", Section~\ref{sec:model1}, as Reviewer 2 pointed out, we specify that workers are risk-neutral expected utility maximizer so that they strategically decide whether or not to accept the task to maximize their quasi-linear utility. 
Finally, in Section~\ref{sec:conclusion}, as a response to {\bf REV2-(2)}, we provide some possible implications
from our analysis considering no worker irrationality to the case with some irrationality such as risk-averse or risk-seeking behaviors.
% the limitation and assumption of our model for worker behavior regarding the risk of getting reward and corresponding prospect theoretic features 
%following the comment {\bf REV2-(2)}.
}

{\bf Revision: Page 3 - Section~\ref{sec:related}, Page 4,5 - Section~\ref{sec:model1}, Page 13,14 - Section~\ref{sec:conclusion}}

\item 

\smallskip
\question{ Include a more thorough discussion of the trade-offs involved in implementing bonus pricing. }
\comments{{\bf REV3-(3),REV3-(5)}}

\smallskip
\answer{
In Section~\ref{sec:model1}, we discuss the complexity of implementing bonus payment at the requester's point of view. We expect that in most cases, the cost incurred by the quality assessment process would not be significant practically. 
%in the worker's point of view, 

We also agree that 
a worker needs to pay additional cost to just interpret and compute the expected bonus payment, which might discourages her participation.
It is an interesting direction of future work.
We however want to note that all the bonus payment schemes which we consider in this paper are much simpler than auction-based ones, e.g., \cite{complexity:einav2018}.
A further discussion is provided in Section~\ref{sec:conclusion}.
}

{\bf Revision: Page 13,14 - Section~\ref{sec:conclusion}}



% \item 

% \question{ Editorial comments}

% \answer{ We appreciate the reviewers' detailed editorial comments.
% We reflected all of them in the revised draft. 
% }


\end{enumerate}

%\newpage

%{\bf Reviewer 1}\hspace{1cm}
\subsection*{Reviewer 1}
\begin{enumerate}[leftmargin=3.5pt]
\item 
\question{There is no clear of proof how a bonus payment pricing can achieve as well as the performance of personalized pricing. Section 3.1 analyzes the “Price of Agnosticity” between the optimal personalized pricing and common pricing without bonus. And Section 3.2 analyzes the power of bonus payment over common pricing with various profile distributions. However, there is no direct comparison of personalized pricing and bonus payment pricing in the paper.}

\answer{
Our major focus is to analyze if the common pricing protocol with bonus is sufficient for microtask crowdsourcing platform. To do so, we show that the performance of a common pricing equipped with a proper bonus payment is close to the optimal pricing that has both personalization and bonus structure, i.e. optimal personalized pricing. Then, based on the case study, we prove that the bonus payment plays a critical role in making such result so that any common pricing without bonus payment can significantly be poor compared to the optimal pricing.

As suggested, it is interesting to study the impact between personalization-only (without bonus) and bonus-only (common) pricing. We hence discuss it in the last paragraph of Section~\ref{sec:poa1}. 
We observe that one does not dominate the other, but it depends on 
the information about the worker profile. 
% , i.e. on the characteristic of the task and accuracy of the requester's information on worker's profile.
}

{\bf Revision : Abstract, Page 2 - Section~\ref{sec:intro}, Page 8 - Section~\ref{sec:poa1}}

\item 
\smallskip
\question{
The writing can be improved. The literature discussed in Section 1.1 seems not so related to the problem investigated in this paper. Moreover, the word “Agnosticity” doesn’t seem to exist in the Collins Dictionary. Maybe the authors can change the word to “Agnostic” or “Agnosticism”.}

\answer{
Please see {\bf RS-(1)} for the related work section.
We also replace the word "Agnosticity" with "Agnosticism" which appears in Collins Dictionary following the suggestion.
}

{\bf Revision : Page 6 - Section~\ref{sec:poa1}}

\item 
\smallskip
\question{In Section 1, the authors state that a simple and eidetic pricing mechanism is needed for microtask crowdsourcing systems, such as Mturk. And two ideas, including personalized and bonus payment are adopted. Therefore, there is a need to compare the gain of personalized pricing and bonus payment pricing. However, in Section 2.1, the authors claim that “… personalized pricing is often discouraged in practice. Amazon Mechanical-Turk utilizes a common pricing.”. The two statements are conflicted. Whether personalized pricing has been used in microtask crowdsourcing systems? If not, the real-world evaluation at Mturk to compare the efficiency of common pricing and personalized pricing may not be convincing enough.}

\answer{
Personalized pricing is often unavailable or discouraged in real-world platforms including Mturk.
%mainly due to privacy concern on accessing worker history.
This motivates us to study whether the form of common pricing is sufficient for crowdsourcing system.
% , since personalized pricing could be available in some applications, but is sometimes discouraged as in Mturk. 
Our analysis shows the sufficiency of common pricing with bonus payment,
in which the bonus payment is necessary.
In Section~\ref{sec:simulation}, 
the simulation result comparing 
optimal personalized pricing and some common pricing policies 
justifies our theoretical findings. 
As Mturk do not support personalized pricing,
in the real-world experiments, it is not avaialble
to directly compare the optimal personalized and common pricing policies.
In Section~\ref{sec:experiment-setup}, we however provide an indirect comparison supporting our message
by emulating the optimal personalized policy based on the estimated worker profiles from the real-world dataset.
% as follows: 
% % From this, we could indirectly estimate the performance of optimal personalized pricing by the following process:
% (i) we post some redundant tasks, that are not used in evaluation, with various base payments but no bonus payment, (ii) estimate the worker's cost and quality distributions based on those tasks, and (iii) finally compute the performance of optimal personalized pricing in brute-force manner using the estimated distributions.

}

{\bf Revision : Abstract, Page 2 - Section~\ref{sec:intro}}

\item 
\smallskip
\question{The submission had been posted on arvix https://arxiv.org/abs/1804.03178. Since all the authors' information are there clearly, this has violated the anonymity requirement.}

\answer{
We apologize for the inconvenience. 
We however double-checked that the anonymity requirement in the submission guideline allows posting on Arxiv. 
% We will consider refreshing the submission on Arxiv to prevent further concerns.
}

\end{enumerate}



%\newpage

%{\bf Reviewer 2}\hspace{1cm}
\subsection*{Reviewer 2}
\begin{enumerate}[leftmargin=3.5pt]
\item 
\question{The paper is quite readable, but the motivation of the common pricing protocol can be improved. There are already earlier work on such kind of common pricing strategy or price bidding scheme being analyzed for cloud computing resources and crowdsourcing problems that were pretty extensive, and insights obtained via the game-theoretic approach in this paper be naturally integrated with some of these earlier work. For example, the paper highlighted the importance of "efficient common pricing scheme", in which individual user can strategically maximizes her individual expected payoff. Earlier similar work for Amazon cloud bidding would be called "spot pricing". For example, see recent ones in:

1) L. Zheng et al, How to Bid the Cloud?, ACM SIGCOMM 2015 2) L. Zheng et al, On the Viability of a Cloud Virtual Service Provider, ACM SIGMETRICS 2016 that demonstrated user profiling, essentially capturing individual user profile to guess a common spot price for bidding to maximize system performance. These prior work would similarly analyze the profile distribution regimes in order to determine the optimal structure of common pricing policies, similarly to how the profile distribution in this paper can be interpreted as a consequence developed by the characteristic of task the requester is trying to solve along with the corresponding behavior of the workers. The game-theoretic nature with Price of Agnoistic can thus have optimization-theoretic implications on the pricing policies with respect to the requester’s task.}

\answer{
We thank you for the insightful comment and the related works.
We refer you to {\bf RS-(1)} and Section~\ref{sec:related} for a discussion about the relation between our work and the mentioned works
%, in which we integrate all the commented papers in Section~\ref{sec:related}
along with some additional works in ride sharing platforms. 
% We agree that the Price-of-Agnosticism and common pricing protocol have an optimization-theoretic implications with respect to the characteristic of requester's task, and it would be an interesting research direction.
}

{\bf Revision : Page 3 - Section~\ref{sec:related}}

\item 
\smallskip
\question{The analysis on the difference between different bonus payment with a common pricing to create tensions, in which if the requester sets high base and low bonus, it may fail to recruit high-quality users leading to only low-cost users may be fleshed out in more details to determine the threshold for the cost that the users can tolerate. It can also be the case that low-cost users may be fewer than what the requester needs to finish the task. On the other hand, if bonus is set too high with low base, it can lead to the presence of more opportunistic users and this part deserves more technical analysis to distinguish the difference between high-quality users and the number of opportunistic users who may be low-quality in nature. Thus, there is a need to provide more analysis on more sophisticated virtual payment mode beyond the base and bonus payments while satisfying the budget constraint.}

\answer{
%Please see {\bf RS-(3)}.
As you mentioned, it is risky to set a high base payment due to the existence of opportunistic workers (or cherry-pickers). This coincides with the choice of common pricing in our analysis, which has only bonus payment, i.e., no base payment. We however want to note that in our experiment, such an issue from opportunistic workers is negligible as {\bf $0.7$-base} shows fair efficiency.

In addition, it is necessary and interesting to
consider irrational workers showing 
risk-seeking or risk-averse behaviors. 
We added a discussion about extending our work
to the case with such irrational workers, in which we believe
the power of bonus will be reinforced
as the worker's irrationality implies an opportunity
to improve budget-efficiency for task requester.
% Section~\ref{sec:conclusion}, we discuss the extension of our work to integrate the irrational worker's behaviors, especially their risk-averse and risk-seeking behaviors in prospect theory.
% In our understanding, two concerns are being pointed out: (i)
% there can be risk-seeking or risk-averse behaviors
% which are irrational;
% % opportunistic workers who accept the high-bonus task even if the cost of participating is
% % her expected utility is below the cost (or risk-averse behavior of workers otherwise),
% (ii) when the requester sets high-base and low-bonus, she might not be able to recruit high-quality workers due to low-cost low-quality workers before the arrival of high quality users.
% For the first concern, in Section~\ref{sec:conclusion}, we discuss the extension of our work to integrate the irrational worker's behaviors, especially their risk-averse and risk-seeking behaviors in prospect theory.
% For the second one, if the eventual number of high-quality worker is enough to exhaust the budget, a smart common pricing would sets the high-bonus and low-base to recruit the high-quality workers only. If it is not the case, any pricing, including personalized one, would admit to recruit all the high-quality workers, and also some of low-cost low-quality workers. Since it is impossible to selectively recruit such low-cost low-quality workers for common pricing, it may fail to recruit all the high quality workers if many low-cost low-quality workers arrive before them. To handle this issue, we adopt the concept of budget approximation ratio, and analyze that if some amounts of budget is added, a smart common pricing is able to asymptotically achieve the utility of optimal personalized pricing.
}

{\bf Revision : Page 13 - Section~\ref{sec:conclusion}}

\end{enumerate}



%{\bf Reviewer 3}\hspace{1cm}
\subsection*{Reviewer 3}
\begin{enumerate}[leftmargin=3.5pt]
% \item 
% \smallskip
% \question{The explanation of budget and costs, in the last paragraph of Section 1.1 is not clear.  }

% \answer{In the revised draft, we clarify the explanation of budget and cost in Section 1, in particular when we first introduce them.}

% {\bf Revision : Page 1, Section 1}

\item 
\smallskip
\question{
I am not sure calling this "bonus" pricing is the best terminology - maybe "quality-based pricing" would better.}

\answer{ 
As suggested, we have re-named it from "bonus-based pricing" to "quality-based pricing" in Section~\ref{sec:model1}, 
while for clarity, we use "bonus payment" apart from "base payment" in the quality-based pricing.
%, to emphasize the quality-dependent terms in quality-based pricing function.
}

{\bf Revision : Page 4 - Section~\ref{sec:model1}}


\item 
\smallskip
\question{In many cases the quality from a worker will depend on the effort exerted by a worked - which is not modeled here (this has been studied in some of the literature) - I think it is fine to not address that here, but do think it would be good to comment on this in more detail.}

\answer{
In Section~\ref{sec:related}, we added a new paragraph on "Quality-based pricing and strategic behavior of workers" to discuss on the comments, in which 
we introduce some related works considering the dependence of worker's quality on her effort or cost, and we discuss 
how our model differs from them with 
some other works supportive of our assumption.
}

{\bf Revision : Page 3 - Section~\ref{sec:related}, Page 4 - Section~\ref{sec:model}}

\item 
\smallskip
\question{Determining the ex post quality is not always possible or easy depending on the crowdsourcing tasks - it would be good to comment on this.}

\answer{
In Section~\ref{sec:model1} and~\ref{sec:conclusion}, we discuss how the assessment of worker quality can be executed in practice.
We remark that in most cases, task requester anyway performs a denoising process to obtain clean labels, in which worker quality can be simply given by comparison between the denoised labels and worker's responses, or as a part of the denoising process.
We refer {\bf RS-(3),(4)} for detailed discussion. 
}

{\bf Revision : Page 4 - Section~\ref{sec:model1}, Page 13,14 - Section~\ref{sec:conclusion}}

\item 
\smallskip
\question{in Theorem 2 - you should indicate what scaling you are considering - I assume this is as n grows?
}

\answer{
Your understanding is correct. The number of workers $n$ is increasing.
For clarity,
we explicitly describe which asymptotic regime is being considered.
% factor, i.e. the number of workers $n$, in the above of Theorem~\ref{thm:ex_post}.
}

{\bf Revision : Page 7, Section~\ref{sec:poa1}}

\item 
\smallskip
\question{One of the main reasons for using posted pricing versus e.g. running an auction is the simplicity of the mechanism - however when "bonus pricing" is used this re-introduces some complexity as both from the users point of view as they have to account for the bonus when deciding whether to accept the tasks and for the platform as it has to estimate the quality and the quality distribution. The use of more structured policies in the numerical experiments partially addresses this but I thought the paper could have done a better job of discussing these trade-offs.}

\answer{
In Section~\ref{sec:model1}, we discuss the complexity of implementing bonus payment at the requester's point of view. As we also said in {\bf REV3-(3)}, 
we expect that in most cases, the cost incurred by the quality assessment process would not be significant practically. 
%in the worker's point of view, 

We also agree that 
a worker needs to pay additional cost to just interpret and compute the expected bonus payment, which might discourages her participation.
It is an interesting direction of future work.
We however want to note that all the bonus payment schemes which we consider in this paper are much simpler than auction-based ones, e.g., \cite{complexity:einav2018}.
A further discussion is provided in Section~\ref{sec:conclusion}.
% and believe that this would be an interesting research direction. As an evidence, in Figure~\ref{fig:exp}\subref{fig:num-worker}, we find that {\bf linear} and {\bf $0.7$-base} engaged more participants than {\bf $50\%$-thre} and {\bf $90\%$-thre} due to their relative simplicity.

% We agree that quality-based pricing increases the complexity to both of task requester and workers,
% and believe that integrating the cost incurred by the increased complexity would be an  

% Please see {\bf RS-(4)}. In Section~\ref{sec:eval}, we added some experimental results, Figure~\ref{fig:exp}\subref{fig:num-worker} and~\ref{fig:exp}\subref{fig:num-worker-by-budget}, and discuss on the trade-off between the complexity of pricing structure and corresponding utility. 
% As we discussed in Section~\ref{sec:eval}, we observe that the participation rate does not decrease in significant manner, which supports that quality-based pricing mechanism actually increases the complexity of the mechanism in terms of the workers, but the amount might be small since the workers do not tend to avoid it in special.
% Secondly in terms of the requester's increased complexity, as discussed in {\bf RS-(4)}, we believe that since inferring the ground truth answer of the task by estimating the worker's quality is the main objective of the requester, crowdsourcing requester would basically maintain a quality estimation process directly~\cite{Inference:4,Inference:5} or indirectly~\cite{deep_crowds}, and hence quality-based pricing would be more feasible and less costly in practice.
% We also agree that considering a cost of the requester to embed a quality estimation process in the model would be an interesting research direction.
}

{\bf Revision : Page 4 - Section~\ref{sec:model1}, Page 13, 14 - Section~\ref{sec:conclusion}}


\end{enumerate}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "response_main"
%%% End:

